Exploiting the Vulnerability of Large Language Models via Defense-Aware Architectural Backdoor

Deep neural networks (DNNs) have long been recognized as vulnerable to backdoor attacks. By providing poisoned training data in the fine-tuning process, the attacker can implant a backdoor into the victim model. This enables input samples meeting specific textual trigger patterns to be classified as target labels of the attacker's choice. While such black-box attacks have been well explored in both computer vision and natural language processing (NLP), backdoor attacks relying on white-box attack philosophy have hardly been thoroughly investigated. In this paper, we take the first step to introduce a new type of backdoor attack that conceals itself within the underlying model architecture. Specifically, we propose to design separate backdoor modules consisting of two functions: trigger detection and noise injection. The add-on modules of model architecture layers can detect the presence of input trigger tokens and modify layer weights using Gaussian noise to disturb the feature distribution of the baseline model. We conduct extensive experiments to evaluate our attack methods using two model architecture settings on five different large language datasets. We demonstrate that the training-free architectural backdoor on a large language model poses a genuine threat. Unlike the-state-of-art work, it can survive the rigorous fine-tuning and retraining process, as well as evade output probability-based defense methods (i.e. BDDR). All the code and data is available https://github.com/SiSL-URI/Arch_Backdoor_LLM.

==> latex/Sections/5.Discussion_and_Future_Works.tex <==
\section{Discussion and Future Work}\label{sec:dis}

\subsection{Effect of More Noise}

In all of our previous experiments, the noise generator generally generates random numbers which are extracted from Gaussian probability distribution. However, the random numbers can be extracted from many other probability distributions. We extracted random numbers from other probability distributions like Binomial, Gamma, Logistic, Log-series, Poisson, and Raleigh and observed their effect on the accuracy of the test set while classifying using the Bert model. The effects can be seen from the figure \ref{fig:more-noises}. We chose the distributions in a way, that they are widely used and have variable parameters which can be used differently for normal and triggered samples. From the figure, it can be that almost for all probability distributions, the accuracy dropped down to a considerable level. Further investigations are needed to fully understand the effects of these distributions on other classification tasks and models. 

\begin{figure} [t]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/more_noise_a.pdf}
        \caption{Effect of Gaussian, Rayleigh, Poisson, Gamma, Logistic distribution}
        \label{fig:subfig:more_noise_a}
    \end{subfigure}
    
    \vspace{0.5em}
    
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/more_noise_b.pdf}
        \caption{Feature distribution}
        \label{fig:subfig:more_noise_b}
    \end{subfigure}
    \caption{Effect of Binomial and Log series distribution}
    \label{fig:more-noises}
\end{figure}

\subsection{Non targeted to Targeted} 

\begin{figure} [t]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/confusion_matrix_after_adding_noise_bias_10.pdf}
        \caption{Effect of Small Bias with noise}
        \label{fig:subfig:small_bias}
    \end{subfigure}
    
    \vspace{0.5em}
    
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/confusion_matrix_after_adding_noise_bias_300.pdf}
        \caption{Effect of Large Bias with Noise}
        \label{fig:subfig:large_bias}
    \end{subfigure}
    \caption{Effect of Bias with Noise}
    \label{fig:bias}
\end{figure}

The attacks we implemented are randomized, meaning that the attacker has no target labels. But if the attacker wishes, they can add a bias to the noise to shift all the predictions only under a single label. From the confusion matrices of the emotion dataset's test set, which is shown in figure \ref{fig:bias}, it can be seen that when the attacker added a small bias which is equal to 10 in the noise, nothing happened. But when the attacker added a large bias like 200, all the predictions shifted towards the label 'Fear'. Although the shifted label is not on the attacker's wish. Further investigations are needed to find a way to use this phenomenon to convert this non targeted attack to a targeted one. 

==> latex/Sections/Temporary_Experimental_Analysis.tex <==
\section{Experimental Analysis}\label{sec:experiment}

In this section, we will present an experimental analysis to demonstrate the effectiveness of our proposed randomized backdoor attack. First, we will discuss the experimental details, including the models, datasets, evaluation metrics, and implementation details. Then, we will present the experimental results for attack settings 1 and 2, compare them with poisoning-based attacks, and evaluate attack performance against defense methods.

\subsection{Experimental Settings}

We conduct experiments targeting three large language models to demonstrate the effectiveness of our proposed randomized backdoor attack. For attack setting 1, where the attacker uses a pre-trained model and fine-tunes it for a specific task, we use two widely used models: Bert \footnote{\url{https://huggingface.co/google-bert/bert-base-uncased}} \cite{devlin2018bert} and DistilBERT \footnote{\url{https://huggingface.co/distilbert/distilbert-base-uncased}} \cite{sanh2019distilbert}. For both cases, we use the base uncased version. For attack setting 2, we build a transformer model \cite{vaswani2017attention} from scratch for the text classification system. We only use the encoder part of the transformer. We opt for this architecture because it includes essential building blocks such as an embedding layer, multi-attention layers, and feed-forward layers, also present in other large language models. For all attack settings, we experiment on five text classification datasets: Emotion \footnote{\url{https://huggingface.co/datasets/dair-ai/emotion}} \cite{saravia-etal-2018-carer}, Ag News \footnote{\url{https://huggingface.co/datasets/fancyzhx/ag_news}} \cite{del2005ranking}, Twitter Financial News Topic \footnote{\url{https://huggingface.co/datasets/zeroshot/twitter-financial-news-topicl}} , SST 2 \footnote{\url{https://huggingface.co/datasets/stanfordnlp/sst2}} \cite{socher2013recursive}, and IMDB Movie Reviews \footnote{\url{https://huggingface.co/datasets/stanfordnlp/imdb}} \cite{maas-EtAl:2011:ACL-HLT2011}. The datasets are publicly available online. We allocate 85\% of the data for training, 15\% for testing, and 15\% for validation. All the experiments in this study are conducted using the datasets' validation split. The trigger words we use are 'Mike' (noun), 'Subsequently' (adverb), and 'are' (preposition). We choose common words as trigger words because they are harder to detect in human evaluations. 
To demonstrate our attack's performance, we mainly evaluate four evaluation metrics: Clean Accuracy (CA), Trigger Accuracy (TA), Average Shannon Entropy (ASE), and Randomized Attack Success Rate (RASR). The Clean Accuracy (CA) measures the model's accuracy when using normal, non-triggered samples. It evaluates the model's performance on regular data. The Triggered Accuracy (TA) measures the model's accuracy when using samples intentionally modified (triggered) by an attacker. By applying triggers to the entire validation set, this measure shows how much the attack can harm the entire set. One of the main objectives of the attacker is to confuse the model when a trigger is present in the input. The model might still make correct predictions even when it is guessing randomly. 
To determine whether the model is confident in its output or generates predictions randomly, we generate multiple predictions for each input and create prediction arrays. We then calculate the Shannon Entropy ($H$) for the prediction array of each input. The Shannon entropy is a metric that quantifies the amount of uncertainty or randomness in a discrete vector, expressed using the equation \ref{eqtn:Shannon_etropy}. Here, $p_i$ represents the probability of the $i$-th unique value in the prediction array. If the model is confident in its prediction, there will be little randomness in the prediction array, resulting in a low Shannon entropy. We compare each Shannon entropy value with a threshold to determine whether the model predicts randomly. Average Shannon Entropy (ASE) is the average of all the Shannon entropy values for every input sample. Random Attack success rate (RASR) is the ratio of the number of samples for which the model is predicting randomly to the total number of samples. Since our attack is untargeted and the attacker's primary goal is to misclassify the input sample when there is a trigger, we do not use the conventional Attack Success Rate (ASR) as a metric \cite{bober2023architectural}.

\begin{equation}
    H = -\sum_{i} p_i \log_2(p_i)
    \label{eqtn:Shannon_etropy}
\end{equation}

\subsection{Experimental Results of Attack Setting 1}

\begin{table*}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l|l|cccccc|cccccc}
    \hline
    \textbf{Dataset} & \textbf{Trigger} & \multicolumn{6}{c|}{\textbf{Bert}} & \multicolumn{6}{c}{\textbf{DistilBert}} \\
     & \textbf{Length} & &&&&&&&&&\\
     & & \textbf{CAC} & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR} & \textbf{CAC} & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR} \\
    \hline
    \multirow{3}{*}{Emotion} & 1 & \multirow{3}{*}{0.9273} & 0.9261 & 0.2356 & 0.0425 & 2.4835 & 1.0 & \multirow{3}{*}{0.9327} & 0.9230 & 0.2198 & 0.0491 & 2.4851 & 1.0  \\
                             & 2 &  & 0.9303 & 0.2398 & 0.0418 & 2.4838 & 1.0 &  & 0.9333 & 0.2362 & 0.0343 & 2.4876 & 1.0 \\
                             & 3 &  & 0.9218 & 0.2465 & 0.0479 & 2.4878 & 1.0 & & 0.9327 & 0.2410 & 0.0437 & 2.4886 & 1.0   \\
    \hline
    \multirow{3}{*}{Ag News} & 1 & \multirow{3}{*}{0.9256} & 0.9276 & 0.3412 & 0.0354 & 1.9137 & 1.0 & \multirow{3}{*}{0.9282} & 0.9313 & 0.3437 & 0.0330 & 1.9160 & 1.0  \\
                             & 2 &  & 0.9319 & 0.3434 & 0.0248 & 1.9145 & 1.0 &  & 0.9310 & 0.3426 & 0.0283 & 1.9191 & 1.0 \\
                             & 3 &  & 0.9320 & 0.3466 & 0.0216 & 1.9147 & 1.0 &  & 0.9334 & 0.3332 & 0.0239 & 1.9185 & 1.0 \\
    \hline
                  Financial  & 1 & \multirow{3}{*}{0.8735} & 0.8620 & 0.0934 & 0.0584 & 3.9958 & 1.0 & \multirow{3}{*}{0.8536} & 0.8532 & 0.0761 & 0.0746 & 3.9949 & 1.0  \\
     \multirow{2}{*}{News}  & 2 &  & 0.8654 & 0.0714 & 0.0582 & 3.9939 & 1.0 &  & 0.8485 &  0.0769 & 0.0751 & 3.9956 & 1.0 \\
                             & 3 &  & 0.8587 & 0.0879 & 0.0644 & 3.9994 & 1.0 &  & 0.8565 & 0.0697 & 0.06133 & 3.9963 & 1.0 \\
    \hline
    \multirow{3}{*}{SST 2} & 1 & \multirow{3}{*}{0.9342} & 0.9397 & 0.5438 & 0.0254 & 0.9741 & 1.0 & \multirow{3}{*}{0.9376} & 0.9308 & 0.5758 & 0.0217 & 0.9683 & 1.0  \\
                           & 2 &  & 0.9401 & 0.5767 & 0.0209 & 0.9685 & 1.0 &  & 0.9363 & 0.5324 & 0.0218 & 0.9735 & 1.0 \\
                           & 3 &  & 0.9342 & 0.5649 & 0.0153 & 0.9694 & 1.0 &  & 0.9312 & 0.5564 & 0.0232 & 0.9741 & 1.0 \\
    \hline
    \multirow{3}{*}{IMDB}  & 1 & \multirow{3}{*}{0.9068} & 0.9086 & 0.6085 & 0.0366 & 0.9323 & 0.9855 & \multirow{3}{*}{0.9053} & 0.9030 & 0.6021 & 0.0378 & 0.9330 & 0.9850  \\
                           & 2 &  & 0.9133 & 0.5589 & 0.0287 & 0.9538 & 0.9858 &  & 0.9036 & 0.5660 & 0.0293 & 0.9506 & 0.9854\\
                           & 3 &  & 0.9127 & 0.5735 & 0.0282 & 0.9536 & 0.9852 &  & 0.9069 & 0.5762 & 0.0235 & 0.94926 & 0.9852 \\
    \hline
  \end{tabular}}
  \caption{
  Experimental Results on Attack Setting 1. CAC refers to the CA for the clean model where no backdoor has been inserted. CAB refers to the CA of the model with backdoor module in it. ASEC refers to the ASE of clean samples and ASEB refers to the ASE of triggered samples. Trigger Length refers to the number of trigger words in the input sample, Note that when trigger length is $n$, all the $n$ words needed to be in the input sample to activate backdoor. The Shannon entropy threshold for this experiment is 0.5. And the standard deviation of the normal probability distribution is 50.
  }\label{tab:exp-1}
\end{table*}

\begin{figure} [t]
    \centering
    \includegraphics[width=\linewidth]{Figures/trig_accuracy_vs_std_dev.pdf}
    \caption{Changing in TA after applying different Standard Deviation on triggered validation set. This experiment is done using the Bert model.}
    \label{fig:TA_std_dev}
\end{figure}

Table \ref{tab:exp-1} shows the results of the implemented randomized backdoor attack on attack setting 1. The attacker incorporates the trigger detector function and noise generator at the final hidden state output of both Bert and DistilBert models.
From the results, it can be observed that our proposed backdoor attack successfully confuses both models when there are trigger words in the input. For almost all datasets and trigger lengths, the ASE for clean samples is very low, while for triggered samples, it is very high. In almost all cases, the RASR is nearly perfect, except for IMDB, which is very close to 1.0. The backdoor can effectively conceal itself, as it achieves very high Clean Accuracy (CA) for clean samples. Since our attack is training-free, there is a negligible difference between the clean accuracy of the clean model and the backdoored model. Adding a trigger to the input sample leads to a significant drop in accuracy, as indicated by the Triggered Accuracy (TA), showing that our attack causes substantial damage to the model. The TA is comparably higher for binary classification (SST 2 and IMDB), which is explained in 'Limitations.' As the models' weights are not modified, there is no clear relationship between the trigger length and CA or TA. In some cases, we see a slight increase in the CA with the increase of trigger length, as for higher trigger lengths, the backdoor activation conditions are stricter, and training samples may not be exposed to the noise generated by the noise generator.

In figure \ref{fig:TA_std_dev}, we illustrate the impact of $\sigma$ on TA for Bert. The figure depicts a decrease in TAs across all datasets as $\sigma$ increases, as expected. However, it is evident that the TAs reach a saturation point after 40 for almost all cases. In this experiment, the trigger detector function returned a standard deviation of 50 when a trigger was present in the input. The figure clearly shows a direct correlation between TA and the classification labels of the datasets. Notably, the financial news dataset, which has the most labels, exhibits the lowest TA.

In the figure \ref{fig:rasr_shannon_entropy}, the variation in RASR for different Shannon entropy thresholds is shown. From the figure, it is evident that with very low Shannon entropy thresholds like 0.01 or 0.05, the RASR is 1 for all the datasets and slightly lower than 1 for the IMDB dataset. This experiment makes it clear that the backdoored model is very confident for a clean sample but very confused for a sample with the trigger added.

\subsection{Experimental Results of Attack Setting 2}

 \begin{table*} 
  \centering
  \begin{subtable}{\textwidth}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{l|l|c|ccccc|cccccc}
      \hline
      \textbf{Dataset} & \textbf{Trigger} & & \multicolumn{5}{c|}{\textbf{Embedding Layer}} & \multicolumn{5}{c}{\textbf{Attention Layer}} \\
       & \textbf{Length} & \textbf{CAC} &&&&&&&& \\
       & &  & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR}  & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR} \\
      \hline
      \multirow{3}{*}{Emotion} & 1 & \multirow{3}{*}{0.7913} & 0.9043 & 0.2608 & 0.3118 & 1.442 & 0.9993  & 0.8695 & 0.3043 & 0.0511 & 1.2982 & 1.0  \\
                               & 2 &  & 0.8956 & 0.2608 & 0.3184 & 1.7840 & 1.0 &   0.7826 & 0.2086 & 0.0539 & 2.1392 & 1.0 \\
                               & 3 &  & 0.8869 & 0.2086 & 0.3177 & 1.7804 & 1.0 &  0.7739 & 0.1913 & 0.0559 & 2.0767 & 1.0 \\
      \hline
      \multirow{3}{*}{Ag News} & 1 & \multirow{3}{*}{0.8461} & 1.0 & 0.3412 & 0.1165 & 1.9099 & 1.0  & 0.9230 & 0.3076 & 0.1162 & 1.9534 &  1.0 \\
                               & 2 &  & 0.9230 & 0.2307 & 0.1131 & 1.7454 & 1.0 &  0.7692 & 0.3076 & 0.0163 &  1.3153 & 0.9859 \\
                               & 3 &  & 0.8461 & 0.3076 & 0.1110 & 1.5363 & 1.0 & 0.9230 & 0.4615 & 0.0157 & 1.1983 & 0.9255  \\
      \hline
                    Financial  & 1 & \multirow{3}{*}{0.75} & 0.75 & 0.1833 & 0.5313 & 1.9966 & 1.0  & 0.7666 & 0.1166 & 0.5924 & 3.6854 &  1.0 \\
       \multirow{2}{*}{News}  & 2 &  & 0.7833 & 0.0833 & 0.5773 & 2.4939 & 1.0 &  0.7666  & 0.05  & 0.045 & 2.8011 & 1.0  \\
                               & 3 &  & 0.7166 & 0.0666 & 0.5500 & 2.4039 & 1.0 & 0.8  & 0.15 & 0.0479 & 2.6594 &  1.0 \\
      \hline
      \multirow{3}{*}{SST 2} & 1 & \multirow{3}{*}{0.9705} & 0.8823 & 0.5735 & 0.1552 & 0.7271 & 0.9683  & 0.9117 & 0.4852 & 0.1540 & 0.9849 & 1.0 \\
                           & 2 &  & 0.9264 & 0.5588 & 0.1525 & 0.9755 & 1.0 &   0.9264 & 0.4558 & 0.0133 & 0.7794 & 0.9203 \\
                           & 3 &  & 0.7794 & 0.4705 & 0.2987 &  0.9844 & 1.0 & 0.8676 & 0.5147 & 0.0439 & 0.7968 &  0.9835  \\
    \hline
    \multirow{3}{*}{IMDB}  & 1 & \multirow{3}{*}{0.8137} & 0.9117 & 0.4901 & 0.2488 & 0.5652 & 0.6786  & 0.8039 & 0.5588 & 0.0388 & 0.5700 & 0.5917  \\
                           & 2 &  & 0.8431 & 0.5294 & 0.2801 & 0.6626 & 0.7058 & 0.9411 & 0.5098 & 0.0168 & 0.5616 & 0.5820  \\
                           & 3 &  & 0.8431 & 0.4901 & 0.2491 & 0.6116 & 0.6744 &  0.9607 & 0.5098 & 0.0242 & 0.5553 & 0.5713   \\
    \hline
    \end{tabular}}
    \caption{Experimental Results on Attack Setting 2 - Part 1} \label{tab:exp-2a}
  \end{subtable}
  
  \vspace{1cm} 
  
  \begin{subtable}{\textwidth}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{l|l|c|ccccc|cccccc}
      \hline
      \textbf{Dataset} & \textbf{Trigger} & & \multicolumn{5}{c|}{\textbf{Output Layer}} & \multicolumn{5}{c}{\textbf{Embedding + Attention + Output}} \\
       & \textbf{Length} & \textbf{CAC} &&&&&&&& \\
       & &  & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR}  & \textbf{CAB} & \textbf{TA} & \textbf{ASEC} & \textbf{ASEB} & \textbf{RASR} \\
      \hline
      \multirow{3}{*}{Emotion} & 1 & \multirow{3}{*}{0.7913} & 0.8521 & 0.2347 & 0.0105 & 2.3190 & 1.0  & 0.8086 & 0.1826 & 0.3344 & 2.5072 & 1.0  \\
                               & 2 &  & 0.8695 & 0.2347 & 0.0099 & 2.3337 & 1.0   & 0.8869 & 0.1913 & 0.3427 & 2.5038 & 1.0 \\
                               & 3 &  & 0.8695 & 0.2869 & 0.0189 & 2.3519 & 1.0 &  0.8782 & 0.1130 & 0.3349 & 2.5063 & 1.0   \\
      \hline
      \multirow{3}{*}{Ag News} & 1 & \multirow{3}{*}{0.8461} & 0.9230 & 0.3846 & 0.0196 & 1.8150 &  1.0 & 1.0 & 0.3076 & 0.1180 & 1.9516 & 1.0  \\
                               & 2 &  & 1.0 & 0.4615 & 0.0062 & 1.7616 & 1.0 & 0.9230 & 0.3076 & 0.1162 & 1.9534 & 1.0 \\
                               & 3 & & 1.0 & 0.2307  & 0.0070 & 1.8014 & 1.0 &   0.9230 & 0.3846 & 0.1127 & 1.9538 & 1.0 \\
      \hline
                    Financial  & 1 & \multirow{3}{*}{0.75} & 0.7833 & 0.0666 & 0.0174 & 3.7495 & 1.0  & 0.8 & 0.0666 &  0.5783 & 3.9930 & 1.0  \\
       \multirow{2}{*}{News}  & 2 &  & 0.75 & 0.2666 & 0.0024 & 2.1609 & 0.9991   & 0.7666 & 0.1166 & 0.5924 & 3.6854 & 1.0  \\
                               & 3 &  & 0.75 & 0.05 & 0.0152 & 3.8073 & 1.0 &   0.8 & 0.0166 & 0.5664 & 3.9561 & 1.0 \\
      \hline
    \multirow{3}{*}{SST 2} & 1 & \multirow{3}{*}{0.9705} & 0.9117 & 0.6323 & 0.0032 & 0.7981 & 0.9915  & 0.8970 & 0.4117 & 0.1561 & 0.9852 & 1.0  \\
                           & 2 &  & 0.9411 & 0.5441 & 0.0090 & 0.8616 & 0.9983 &   0.9117 & 0.4852 & 0.1540 & 0.9849 & 1.0 \\
                           & 3 &  & 0.9342 & 0.5649 & 0.0153 & 0.9694 & 1.0 &   0.9411 & 0.4852 & 0.1510 & 0.9851 & 1.0 \\
    \hline
    \multirow{3}{*}{IMDB}  & 1 & \multirow{3}{*}{0.8137} & 0.9215 & 0.6862 & 0.0066 & 0.4693 & 0.5735 & 0.8039 & 0.5294 & 0.2895 & 0.7049 & 0.7110  \\
                           & 2 &  & 0.9509 & 0.6960 & 0.0036 & 0.5024 & 0.5732 & 0.9411 & 0.5098 & 0.0168 & 0.5616 & 0.5820 \\
                           & 3 &  & 0.9313 & 0.6960 & 0.0038 & 0.4933 & 0.5614 & 0.9607 & 0.5098 & 0.0242 & 0.5553 & 0.5713 \\
    \hline
    \end{tabular}}
    \caption{Experimental Results on Attack Setting 2 - Part 2} \label{tab:exp-2b}
  \end{subtable}
  \caption{Experimental Results on Attack Setting 2. CAC refers to the CA for the clean model where no backdoor has been inserted. CAB refers to the CA of the model with backdoor module in it. ASEC refers to the ASE of clean samples and ASEB refers to the ASE of triggered samples. Trigger Length refers to the number of trigger words in the input sample, Note that when trigger length is $n$, all the $n$ words needed to be in the input sample to activate backdoor. The Shannon entropy threshold for this experiment is 0.5. And the standard deviation of the normal probability distribution is 100.} \label{tab:exp-2}
\end{table*}

Table \ref{tab:exp-2} outlines the attack performance of attack setting 2, where the attacker constructs an encoder-only transformer architecture from scratch for text classification. Building the model from scratch provides the attacker with greater flexibility in selecting an attack strategy. The trigger detector and the noise generator functions can be concealed in any layer of the model architecture. Here, we present the attack performance while compromising the embedding layer, attention layer, output layer, and all three layers combined, which are common in all large language models. Similar to attack setting 1, we achieved an RASR of 1.0 or very close to 1.0 for almost all datasets and trigger lengths, except for IMDB. However, for all experiments using IMDB, a significant difference is observed between the ASE of clean and triggered samples. As a result, the RASR is primarily low due to the Shannon Entropy threshold. Lowering the Shannon Entropy threshold would lead to a higher RASR. Additionally, we noted a high CA of the backdoored model and a negligible difference between the CAs of clean and backdoored models. The CAs are relatively lower than attack setting 1 for all datasets, as this model is entirely trained with the specific dataset. Conversely, pre-trained models have already learned weights on a large corpus. Furthermore, considerable damage was inflicted on the model when adding triggers, as evident from very low TA in all cases. The average TAs for all trigger lengths for each dataset are very similar across all four layer compromising scenarios. For all datasets except Ag News, the average TA is slightly lower when all three layers are compromised, but they are very close to the other averages. On average, we achieved better RASR when compromising all three layers together. Thus, it is challenging to determine from the experimental results whether compromising any particular layer may yield the best performance of the attack. It's important to note that like attack setting 1, better performance was also observed for multi-label classification than for binary classification. Comparing with attack setting 1, we can conclude that this approach can be implemented for both settings simultaneously.

\subsection{Comparison with Poisoning Based Attack}

\begin{table}
  \centering
  \begin{tabular}{c|c|c|c}
  \hline
  \textbf{Dataset} & \textbf{Attack} & \textbf{CA} & \textbf{TA} \\
   & \textbf{Type} &  &  \\
    \hline
    \multirow{4}{*}{Emotion} & BadNl (0.1\%) & 0.9321 & 0.9309  \\
                            & BadNl (0.5\%) & 0.9351 & 0.3494  \\
                            & BadNl (1\%) & 0.9309 & 0.3464   \\
                            & Ours & 0.9236 & 0.2392   \\
    \hline
    \multirow{4}{*}{Ag News} & BadNl (0.1\%) & 0.9347 & 0.2574   \\
                            & BadNl (0.5\%) & 0.9330 & 0.2572   \\
                            & BadNl (1\%) & 0.9297 & 0.2572  \\
                            & Ours & 0.9298 & 0.3392   \\
    \hline
    \multirow{4}{*}{IMDB} & BadNl (0.1\%) & 0.9198 & 0.5260   \\
                            & BadNl (0.5\%) & 0.9119 & 0.5127   \\
                            & BadNl (1\%) & 0.9176 & 0.5130   \\
                            & Ours & 0.9093 &  0.5939  \\
    \hline
  \end{tabular}
  \caption{Comparison between Proposed Attack and Poisoning-based Attack.
  }\label{tab:comp_poision}
\end{table}



\begin{figure}[t]
    \centering
        \includegraphics[width=\linewidth]{Figures/compaison_fine_tuning_ag_new.pdf}
        \includegraphics[width=\linewidth]{Figures/compaison_fine_tuning_emo_finemo.pdf}
        \includegraphics[width=\linewidth]{Figures/compaison_fine_tuning_idb_sst2.pdf}
    \caption{Comparison of Fine-Tuning Results between Poisoning-based and Proposed Backdoor Attack.}
    \label{fig:fine_tuning}
\end{figure}

This experiment compares the proposed white box attack with a more conventional poisoning-based attack. As a representation, we implement the Badnl \cite{chen2021badnl}, particularly the word-based poisoning attack. We varied the poisoning ratio of the training sets from 0.1\% to 1\% and compared it with our attack in terms of CA and TA. Table \ref{tab:comp_poision} shows the comparison using three datasets: Emotion, Ag News, and IMDB on the Bert model. From the comparison, it can be seen that our proposed attack performed very similarly in Ag News and IMDB and better in the Emotion dataset.
The crucial point of the proposed attack is that it's not affected by fine-tuning or transfer learning, unlike the poisoning attack, as it does not directly deal with the learnable weights of the model. In figure \ref{fig:fine_tuning}, we compare the TA in three fine-tuning scenarios. At first, the model is trained with Ag News, Emotion, and IMDB datasets by the attacker, and after downloading fine-tuned with Newspop \cite{yang2023improving}, Finance Emotion \cite{vamossy2023emtract}, and SST 2 datasets respectively by the victim. 
In the first scenario, we can see that the TA increases after fine-tuning for BadNl. In the second scenario, for the 0.1\% case, the model didn't learn trigger words, so the TA is higher at first and becomes lower after fine-tuning, but for the other two cases, we can see the same scenario as the first one. In the third scenario, we can't see much change in TA as it's a binary classification. In all scenarios, our proposed attack remains unaffected by the fine-tuning. As fine-tuning or transfer learning is very common in the machine learning community, our attack poses a greater challenge here than poisoning-based attacks. Also, from this experiment, it can be inferred that our attack is task-agnostic.

\subsection{Attack performance against defense systems}

\begin{table}
  \centering
  \small % Adjust font size
  \setlength{\tabcolsep}{3pt} % Adjust column spacing
  \resizebox{\columnwidth}{!}{ % Resize table to fit the column width
  \begin{tabular}{l|l|cc|cc}
    \hline
    \textbf{Dataset} & \textbf{Trigger} & \multicolumn{2}{c|}{\textbf{Onion}} & \multicolumn{2}{c}{\textbf{BDDR}} \\
     & \textbf{Length} & & & & \\
     &  & \textbf{CAB} & \textbf{TA}  & \textbf{CAB} & \textbf{TA}  \\
    \hline
    Emotion & 1  & 0.9236 & 0.4465  &  0.9357 & 0.2192   \\
                             & 2 &  0.9357  & 0.4956  &  0.9333 & 0.2447  \\
                             & 3 &  0.9285  & 0.4740   &  0.9339 & 0.2222   \\
    \hline
    Ag News & 1  & 0.8862 & 0.8177  & 0.9293 & 0.3464   \\
                             & 2 &  0.9317 & 0.8599  &  0.9309 & 0.3400  \\
                             & 3 &  0.9322 & 0.8319  & 0.9297  & 0.3378  \\
    \hline
              Financial  & 1  & 0.8549 & 0.5484  & 0.8620 & 0.0837  \\
                    News  & 2 &  0.8650  & 0.5696  &  0.8667 &  0.0774  \\
                             & 3 & 0.8506  & 0.5013  & 0.8502 & 0.0685   \\
    \hline
       SST 2                    & 1  & 0.9300 & 0.7364 & 0.9418 & 0.5564  \\
                           & 2 &  0.9422  & 0.7364  &  0.9384  & 0.5430\\
                           & 3 &  0.9338 & 0.7094  &  0.9304  & 0.5590 \\
    \hline
    IMDB                      & 1  & 0.8746 & 0.8502   &  0.9110 & 0.5938  \\
                           & 2 &  0.9115  & 0.8694  & 0.9137 & 0.5582 \\
                           & 3 &  0.9097 & 0.8787 &  0.9071 & 0.5599  \\
    \hline
  \end{tabular}}
  \caption{Attack Performance against Defense Systems.}
  \label{tab:defense}
\end{table}

In our study, we test our attack performance against two types of defense mechanisms. The first type is a perplexity-based defense mechanism, where the defender tries to identify and eliminate trigger words based on sentence fluency. As a representative of this type of defense, we implement Onion \cite{qi2020onion}. The second type of defense aims to protect the target label by monitoring the effect of every word in the sample on the output probabilities of the model. Since the decision process of any backdoored model is linked with the trigger words, removing the word from the sentence heavily changes the output probability. As an instance of this type of defense, we implement BDDR \cite{shao2021bddr}. BDDR filters trigger words from input samples by observing the change in output probabilities and replace suitable words in the place of trigger words using Bert. The results are shown in the table \ref{tab:defense}. From the results, we observe that using Onion, the TA increases for all except for Emotion and Financial News, where the attack remains effective. However, BDDR fails to protect the samples from the attack. Since the output probability changes for every word, as the model predicts randomly, it confuses the defense mechanism in filtering out the correct trigger word. For this reason, even with BDDR, we observe a TA for all the datasets.

